Dim Wihl Gat Tun: The Case for Linguistic Expertise in NLP for Underdocumented Languages

Recent progress in NLP is driven by pretrained models leveraging massive datasets and has predominantly benefited the world's political and economic superpowers. Technologically underserved languages are left behind because they lack such resources. Hundreds of underserved languages, nevertheless, have available data sources in the form of interlinear glossed text (IGT) from language documentation efforts. IGT remains underutilized in NLP work, perhaps because its annotations are only semi-structured and often language-specific. With this paper, we make the case that IGT data can be leveraged successfully provided that target language expertise is available. We specifically advocate for collaboration with documentary linguists. Our paper provides a roadmap for successful projects utilizing IGT data: (1) It is essential to define which NLP tasks can be accomplished with the given IGT data and how these will benefit the speech community. (2) Great care and target language expertise is required when converting the data into structured formats commonly employed in NLP. (3) Task-specific and user-specific evaluation can help to ascertain that the tools which are created benefit the target language speech community. We illustrate each step through a case study on developing a morphological reinflection system for the Tsimchianic language Gitksan.

==> edit_2021_11_02/evaluation-3-4.tex <==
\section{Building and Evaluating NLP Models for Underdocumented Languages} \label{sec:eval-challenges}
\label{sec:evaluation}

% In many previous morphological inflection tasks, such as SIGMORPHON’s shared-tasks\cite{}, can reach an average accuracy above 0.9 over the scores of all languages, even for those really underserved languages. Although the good performance of those generic neural systems led research into further steps, Goldman et al\cite{} propose that the evaluation methods used in SIGMORPHON shard tasks is defective: on the one hand, the test data is not challenging enough which includes lemmas in the training set. On the other hand, the data-split is far from the realistic use of those models in the wild \cite{}(Søgaard et al., 2021). Thus, they reconstructed a more difficult dataset where all of test data are unseen lemmas. Under this setting, morphological inflection drops by 30\% macro-average, and up to 95\% in low-resource settings. Following their practice, we decide to adopt their splitting method. 

% Besides using this refined data split for our data evaluation. We further take advantage of data augmentation techniques for the inflection-generating task. The first technique we use is back translation, which is a common practice in machine translation
% in low-resource scenarios. Although it is regarded as a data augmentation technique, no previous work has applied it for morphological inflection under the low-resource circumstance. The second technique we use is data hallucination. We use the monolingual data hallucination method proposed by Neubig et al \cite{}.

% In addition, in order for these technologies to be adopted, we need to have more interpretable models, since neural network models are usually poorly calibrated \cite{} and suffer from overconfidence or good uncertainty estimates problems. Thus, during the model prediction process, we attempt to achieve more accurately estimate the knowledge acquired in those models....
\begin{figure}[!htb]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{edit_2021_11_02/paradigm_num_forms_hist.pdf}
         \caption{}
         \label{fig:paradigm-fullness-dist}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{edit_2021_11_02/paradigm_msd_dist.pdf}
         \caption{}
         \label{fig:msd-dist}
     \end{subfigure}
     \caption{(a) Distribution of the number of MSDs that are filled in a paradigm. (b) Distribution of the number of times an MSD is filled in a paradigm.}
\end{figure}
The previous section described challenges in massaging the IGT data into a format amenable for a computational task, specifically the Paradigm-Cell Filling Problem \citep[PCFP;][]{ackerman2009parts}. Researchers have put forward myriad proposals for optimally solving the PCFP task \citep{Cotterell2017CoNLLSIGMORPHON2S}, but the manner in which these proposals are evaluated have seldom changed. 
NLP models, like those for the PCFP, are typically compared through accuracy on standard benchmarking datasets. Benchmarking supports standard
comparisons of different proposals and provides concrete goals for the research community \citep{Ma2021DynaboardAE}. Obtaining state-of-the-art results on a computational task, however, should not always be the goal for NLP research. In the case of developing digital infrastructure for an underdocumented language, the goals of the research should be designed collaboratively with linguists as well as speech community members. This collaboration will result not only in more practical outcomes for the community \citep{Bird2020DecolonisingSA}, but also more challenging benchmarks for NLP research. We support this claim through our case study.


\noindent \textbf{Dataset skew}. For an automatic morphological inflection system to be beneficial in developing pedagogical resources for Gitksan, it must be able to generalize outside of the training data distribution. Specifically, it must be able to inflect lemmas that were unseen in the training data. Although tremendous progress has been made in morphological inflection in recent years \citep{McCarthy2019TheS2}, especially for low-resource languages \citep{anastasopoulos2019pushing}, \citet{Goldman2021UnsolvingMI} report that true generalization ability in morphological inflection has been vastly overestimated by the standard train/validation/test split for evaluating models. Specifically, they report that when tested exclusively on inflecting lemmas unseen during training, accuracy drops by a macro-average of 35\% and up to 95\% for some acutely low resourced languages on state-of-the-art models. It is precisely in the unobserved-lemma setting where morphological inflection models must perform well for developing pedagogical resources: our paradigm dataset for Gitksan demonstrates that the overwhelming majority of paradigms have very few entries (\Figure{fig:paradigm-fullness-dist}). Similarly, class-imbalance is prevalent in our realistic dataset for an underdocumented language: most labels are attested only a few times (\Figure{fig:msd-dist}). Having end-users (linguists and speech community members) involved in the research forces us to consider realistic evaluations from the outset of the project that more accurately gauge the progress of the research.


\noindent \textbf{Population skew}. Linguistic fieldwork is typically conducted by working with a handful of willing participants; this is not necessarily a representative sample of the speaking community. From working with documentary linguists through the outset of the project, we were acutely aware that the dataset only comprises four speakers that dedicated their time and expertise in serving as language consultants. Since training NLP models only on four speakers risks overfitting to idiosyncrasies of their speech patterns, we developed evaluation schemes to assess this risk. Specifically, we devised leave-one-speaker-out evaluations, training only on inflection data from three speakers while testing on the fourth. This evaluation scheme provides some estimate of the degree to which we are over fitting to a speaker, and prevents harmful overclaims of our model performance. Again, it is necessary to consult with the linguists involved in the documentation to understand the realities of the dataset construction that will inevitably affect our language technologies' performance. 

==> edit_2021_11_02/introduction.tex <==
\section{Introduction}

\todo{MS: Add some discussion on the Haspelmath paper in the intro. We raise similar points in the paper}
\fs{This intro takes too long to get to the point}

Progress\footnote{\textit{Dim wihl gat tun} - ``This is what the people should do''} in NLP research has primarily manifested in tools for the world's political and economic superpowers \citep{blasi2021systematic}, and it
is unclear how we can build more inclusive language technologies. Leveraging multilingual pretrained models has been a fruitful direction: they have led to substantial gains for many low-resource languages which have traditionally suffered from performance issues due to the absence of large annotated training sets. For example, multilingual pretrained languages models like MBART \cite{liu2020multilingual} have enabled training of high-performance neural machine translation systems for many languages where large parallel datasets are unavailable. These new methods have substantially increased the number of speakers who can benefit from NLP applications and NLP research now targets a wider selection of languages than ever before \cite{joshi2020state}.

It is tempting to conclude that this research path will lead to a world where everyone can access NLP applications in their native language. Unfortunately, multilingual pretraining can only take us so far since not all low-resource languages are documented alike. Only a minority of low-resource languages have enough data available to benefit from pretrained language models when leveraging cross-lingual transfer from higher-resourced languages. \newcite{joshi2020state} estimate that approximately 90\% of the world's language have too few available data sources to successfully utilize cross-lingual pretraining, motivating their categorization of these languages as ``left-behinds''.

But should these languages be considered "left-behind" simply because they lack \textbf{off-the-shelf} datasets for cross-lingual pretraining? Consider a language like Gitksan of the Tsimshianic language family. It has the features of a ``left-behind language'': namely, no off-the-shelf datasets whether unlabeled (e.g., Wikipedia articles) nor labeled (e.g., via the LDC repository\footnote{https://catalog.ldc.upenn.edu}).
But speakers and linguists have been collaborating to document the language for more than 50 years, producing hours of speech recordings, carefully curated bilingual dictionaries and wordlists, and several thousand tokens of richly-glossed text \citep{forbesetal2017}.    

\begin{figure}
\glll Ii al'al\Gitg alt\Gitg athl get, [...] \\
            ii CVC-al\Gitg al-t=\Gitg at=hl get \\
            \textsc{ccnj} \textsc{pl}-watch-\textsc{3.ii}=\textsc{report}=\textsc{cn} people \\
            `And they stood by and watched, [...]'
\caption{A line from the Interlinear-Glossed-Text corpus for Gitksan. The first line represents a transcription of the Gitksan utterance, the second line a morphological segmentation, the third line a gloss of the morphemes in the utterance, and the final line an English translation. \fs{The point we want to make with this figure is IGT is richly structured.}}
\label{fig:igt-gitksan-example}
\end{figure}

Artifacts from documentary linguistic efforts are all we have not only for Gitksan but for thousands of languages. Multilingual dictionaries have been produced from documentary efforts for over 1000 languages \citep{Wu2020MultilingualDB}; aligned speech recordings are available for 700+ languages \citep{Black2019CMUWM,Adams2019MassivelyMA,Black2019CMUWM}; and interlinear glossed text is continually generated through language documentation efforts and made available for hundreds of languages in digitized databases \citep{lewis2010developing,xia2016enriching}. For \textit{under-documented}\footnote{By ``under-documented'', we refer to languages with no \textbf{comprehensive} dictionary, grammar, or pedagogical materials.} languages, this language documentation data is all we have to work with as off-the-shelf datasets are very unlikely to materialize in the future. Too many obstacles prohibit the production of off-the-shelf datasets, not least of which is the lack of basic digital infrastructures like standardized writing systems, keyboard layouts, and access to the internet.
Given that the language documentation artifacts are sufficient for building (some) language technologies, as we discuss in \Sectref{sec:nlp-underdocumented}, we believe that the label of ``left-behind'' is inappropriate: further progress can be made for underdocumented languages. 

Yet leveraging language documentation data for building language technology poses considerable challenges and risks that have received little attention in the literature. Language documentation data used in computational applications is largely treated as though it were sanitized, refined (i.e., ``gold'') data that can be used as ground-truth for training and evaluating a computational system: ``the messy and incomplete processes that created the data are hidden from view'' \citep[][and references therein]{bird2020decolonising}. 
An important concern about documentary linguistics datasets, for example, is that they typically comprise speech transcriptions and recordings from only a handful of language consultants from the speech community, dramatically increasing the risk of designing a system that overfits to a specific speaker, age-group, or dialect. 

Although researchers have noted isolated issues with some language documentation datatypes \citep[][inter alia]{moeller2020igt2p,zhao-etal-2020-automatic} like transcription errors, there are no descriptions of the systemic challenges in using language documentation data for NLP applications. \todo{MS: Maybe soften this?} %\todo{Shorten following sentence}
The shrinking number of speakers in many, if not most under-documented languages, provides an urgency to the question of how to best utilize language documentation data in NLP research. NLP methods can speed up language documentation and support language revitalization efforts.

In this work, we present a systematic analysis of the risks and challenges in developing language technologies using language documentation data, specifically Interlinear Glossed Text (IGT) corpora. We focus on IGT since it is the only source of data for many of the world’s languages, and it is the de-facto standard annotation format in language documentation. We perform our analysis of the challenges and risks of leveraging IGT for computational applications through a concrete case study on developing a morphological inflection system for the Gitksan language, starting from glossed text collected by documentary linguists (\Figure{fig:igt-gitksan-example}). 

Through this case study, we argue that building language technology for underdocumented languages must be a collaborative effort between documentary linguists and NLP researchers. In \Sectref{sec:preprocessing}, we describe the roadblocks of preprocessing IGT data for NLP applications that can only be removed through collaboration with linguists. In \Sectref{sec:eval-challenges} \todo{MS: Missing ref}, we describe how collaboration with linguists can assist in constructing practical evaluations of NLP tools that reflects designing for speech communities rather than competing with other NLP researchers. Overall, in accordance with the ACL 2022 theme, our research highlights frequently overlooked challenges and provides concrete recommendations for making meaningful advances in NLP research for underdocumented languages. 

==> edit_2021_11_02/introduction_old.tex <==
\section{Introduction}

Progress\footnote{\textit{Dim wihl gat tun} - ``This is what the people should do''} in NLP research has primarily manifested in tools for the world's political and economic superpowers \citep{blasi2021systematic}; how can we build more inclusive language technologies? A direction that has proved to be fruitful is leveraging multilingual pretrained models; they have lead to substantial gains for many low-resource languages which have traditionally suffered from performance issues due to absence of large annotated training sets. For example, multilingual pretrained languages models like MBART \cite{liu2020multilingual} have enabled training of high-performance neural machine translation systems for many languages where large parallel datasets are unavailable. These new methods have substantially increased the number of speakers who can benefit from NLP applications, and NLP research now targets a wider selection of languages than ever before \cite{joshi2020state}. %{\color{red} Get rid of mentions of unlabeled vs. labeled. Focus on the data quantity.}

It is tempting to conclude that the current development is leading us toward a world where everyone can access NLP applications in their native language. Unfortunately, cross-lingual transfer methods can only take us so far; not all low-resource languages are documented alike. In fact, only a minority of low-resource languages have enough data available to benefit from pretrained language models even when leveraging cross-lingual transfer from higher-resourced languages. \newcite{joshi2020state} estimate that approximately 90\% of the world's language have too few available data sources to successfully utilize cross-lingual pretraining, motivating their categorization of the languages as ``left-behinds''.

% \footnote{\newcite{joshi2020state} divide the world’s languages into six categories according to digital viability and resource-richness. On one end, we have category 5 languages like English and Japanese, where ample unannotated and annotated data are available for training NLP systems. On the other end, we have category 0 languages or the “Left-behinds” where very litle or no data are available, such that it is very unlikely that these languages will benefit from recent advances in low-resource NLP.} %Compounding the lack of data, many of these languages do not have a standardized orthography, or even a writing system. Many also lack digital resources like keyboard layouts mening that large quantities of new data is unlikely to materialize in the near future. 
Although many of these {\it under-documented} languages have small speech communities, they are by no means unimportant. Combined, they have around 1 billion speakers. They also represent a vast linguistic richness and therefore a challenging testing ground for NLP methods. 

% A major problem for NLP research is that many of the category 0 languages have few speakers, no standardized orthography, and no presence on the Internet.  Ethnologue\footnote{www.ethnologue.com} lists more than 7000 languages that are spoken in the world and the vast majority of these have a relatively low populations of speakers.  Ethnologue further estimates that more than 95\% of the world's population speaks one of 306 languages ($\sim$5.6\%) as a first language. The other 94\% of languages have fewer than 1,000,000 speakers each, with more than half of all languages having between 1,000 and 100,000 speakers.  

For the vast majority of under-documented languages, large datasets are unlikely to materialize in the near future. Too many obstacles prohibit this, starting with the lack of basic digital infrastructure like standardized writing systems, keyboard layouts, and access to the internet. Despite these challenges, we argue that the label of ``left-behinds'' for these languages is inappropriate. There is one data source which is available for many of these languages: interlinear glossed text (IGT), which is continually generated in language documentation efforts and is available for hundreds of languages in digitized databases \cite{lewis2010developing,xia2016enriching}. 

IGT is a semi-structured representation typically consisting of 3-4 lines of text. The following is an example by \newcite{forbes-etal-2021-fst} for  Gitksan, one of the Indigenous languages of the Pacific Northwest:

\ex.\glll Ii al'al\Gitg alt\Gitg athl get, [...] \\
            ii CVC-al\Gitg al-t=\Gitg at=hl get \\
            \textsc{ccnj} \textsc{pl}-watch-\textsc{3.ii}=\textsc{report}=\textsc{cn} people \\
            `And they stood by and watched, [...]'%\vspace*{-7pt}

\begin{figure}
\glll Ii al'al\Gitg alt\Gitg athl get, [...] \\
            ii CVC-al\Gitg al-t=\Gitg at=hl get \\
            \textsc{ccnj} \textsc{pl}-watch-\textsc{3.ii}=\textsc{report}=\textsc{cn} people \\
            `And they stood by and watched, [...]'%\vspace*{-7pt}

\caption{Explain IGT}
\end{figure}

The first line represents a transcription of the Gitksan utterance, the second line a  morphological segmentation (with some added normalization), the third line is a gloss of the morphemes in the utterance and the final line an English translation.

IGT represents the only source of  data for many of the world’s languages but utilizing it in NLP research is far from straightforward. Unlike many of the annotated datasets used in NLP, glossed text is not specifically created for computational applications. Instead, it is meant as a guide to clarify the relation between text and a parallel translation. Documentary linguists who produce IGT have a variety of research agendas and varying levels of experience with the language in question, both of which evolve as a documentation project progresses and influence the IGT annotation. For example, morphemes which indicate structural information but are dropped in rapid speech might be annotated in the gloss to present a clearer syntactic picture even though they are not present in the source utterance. This naturally requires in-depth understanding of the language and is, therefore, only possible at later stages in the documentation process.\footnote{Source: personal communication with linguists producing IGTs for Gitksan.} 

Existing computational research leveraging IGTs have treated them as off-the-shelf datasets amenable for NLP tasks like morphological analysis \cite{zamaraeva2016inferring,wax2014automated}, automatic glossing \cite{zhao-etal-2020-automatic,moeller2018automatic}, and paradigm discovery \cite{moeller2020igt2p}. This paper instead presents an in-depth analysis of IGT as a datatype and investigates some of the challenges which are encountered when working with IGT. Due to dwindling speaker numbers of many, if not most under-documented languages, the question of how to best utilize IGT in NLP research is urgent both for language documentation, where automatic methods can lead to speed-up, and for language revitalization, which can benefit from computational methods. We must quickly adapt the NLP workflow involving IGTs to accept the reality of their dynamic evolution.

% do the the shrinking \fs{awkwardly worded this.} \todo{In order for NLP to have an impact in preserving linguistic diversity, we must quickly adapt the NLP workflow involving IGTs to accept the reality of their dynamic evolution}. {\color{purple} Reorder the content. Talk about creating of IGTs first and then bring up related work.}




% Existing work has treated IGTs produced through language documentation as off-the-shelf datasets for training NLP models in tasks including morphological analysis, automatic glossing, and paradigm discovery. This approach entails several assumptions which are unrealistic for a language which is undergoing documentation, not least of which is that the annotations are static and consistent. In fact the entire annotation schema might undergo changes during the documentation process. Furthermore, due to a lack of existing grammars for the target language, glossing labels are frequently surface-oriented meaning that identical morphological exponents which are used in several very divergent functions might be annotated using a single label. This means that annotations cannot be reliably interpreted without substantial domain knowledge concerning the documentation process and the target language itself. This is in stark contrast to higher-resourced languages, where the glossing process can rely on extensive grammatical descriptions of the target language.

Through a case study on developing automatic morphological inflection and analysis tools from in-development IGTs for the Gitksan language, we will discuss how the dynamic nature of linguistic fieldwork has implications for expanding the linguistic diversity represented by NLP research (in accordance with the ACL2022 special theme). We argue that a documentary-linguist-in-the-loop paradigm is essential for every step in developing NLP tools for under-documented languages from task specification (Section 3.1) to evaluation (Section 3.4). In particular, we explain how such a paradigm will:
\begin{itemize}
    \item Help create computational tasks that will provide the most benefit for documenting under-documented languages (Section 4.1)
   \item Ensure robustness of NLP systems for several dialects for under-documented languages (Section 4.2)
   \item Guide research toward more representative/diverse annotation standards for training supervised NLP models (Section 4.3)
   \item Prevent harmful overgeneralization of findings and improve adoption of NLP models for language documentation by using appropriate evaluation methodologies  (Section 4.4)

\end{itemize}
%{\color{red} Exapnd Gitksan content in this paragraph. The related work needs to make sense after reading this paragraph}

% Although Ethnologue\footnote{www.ethnologue.com} lists more than 7000 languages that are spoken in the world, the vast majority have a relatively low population of speakers.  Ethnologue further estimates that more than 95\% of the world's population speaks one of 306 languages (~5.6\%).  The other 94\% of languages have fewer than 1,000,000 speakers, with more than half of all languages having between 1,000 and 100,000 speakers.  In an era of big data, it is simply not possible to create linguistic data as fast as more-commonly spoken languages.  As we become more and more dependent upon computational tools, there is a danger that a lack of automatic language tools may lead speakers away from certain languages, further exacerbating the problem.  However, working with documentary linguists, who themselves often work very closely with language communities, it may be possible to accelerate the creation of these resources.
% % It's been estimated that nearly 90$\%$ of internet usage occurs in just 10 languages \cite{https://www.visualcapitalist.com/the-most-used-languages-on-the-internet/}, making up only about 50$\%$ of the world's population.  Some of this dominance can be attributed to the economic and political power of the countries where these languages are spoken, and this influence has also made these languages popular second languages.  However, many of the world's languages simply do not have computational tools that would allow for a significant digital presence.  

% The progress in NLP research has accelerated rapidly, primarily due to advances in machine learning for massive datasets. Although this progress has primarily manifested in tools for the world's political and economic superpowers \citep{blasi2021systematic}, where data is abundant, an emergent body of research demonstrates machine-learning techniques could play a significant role in accelerating language documentation and revitalization. 
% In supporting language documentation efforts, researchers have expended significant effort in developing sophisticated models for computational tasks in the low-resource settings that are typical of language documentation. \todo{These models are of practical importance in developing digital infrastructure like keyboard completion, etc as well as pedagogical resources for supporting lagnuage revitalization}.
% To name only a few: researchers have developed models for automatic morphological inflection \citep{anastasopoulos2019pushing,lane2020bootstrapping}, machine translation (\todo{add citation(s) for Nicolai et al., others}), and spoken term recognition (\todo{Anastsaopolous et al., Bird et al}). 

% \fs{We could use some more related work here}
% Of particular importance to us is computational efforts to automatically extract information from 
% and create interlinear glossed texts (IGTs). Given that data elicited through linguistic fieldwork
% is typically transcribed and annotated through in IGT format (\todo{give example in Gitksan?}), IGT data
% is available for many underresourced languages that are actively undergoing documentation (\todo{Moeller et al., 2020}). Effectively processing IGT data to accelerate language documentation is of great importance for this subfield. Existing work on automatically extracting information from IGTs has looked at extracting paradigms from the data (\todo{Moeller et al., 2020}). Existing work has also looked at automatically producing IGTs for unannotated data \todo{Cite Hulden and Moeller; Neubig and Anastasopolous; and Bender et al.)}. 

% \fs{This paragraph is incomplete (more incomplete than the others)}
% Existing work has treated IGTs produced through language documentation as static, raw datasets for training NLP models. 
% \todo{What sort of assumptions and how do they connect to our outlines for Sections 3.1 to 3.4}.
% In particular, existing work has assumed that the  
% Unfortunately, these assumptions are not at all warranted given the dynamic nature of language documentation and fieldwork. 

% {\color{red} Existing work has treated IGTs produced through language documentation as static, raw datasets for training NLP models. This approach entails several assumptions which are unrealistic for a language which is undergoing documentation: The annotations are all but static. In fact the entire annotation schema might undergo changes during the documentation process. Furthermore, due to a lack of existing grammars for the target language, glossing labels are frequently surface-oriented meaning that the an affix which is used in several very divergent functions might be annotated using a single label. This means that annotations cannot be reliably interpreted without substantial domain knowledge concerning the documentation process and the target language itself. This is in stark contrast to higher-resourced languages, where the glossing process can rely on extensive grammatical descriptions of the target language.}

% Through a case study on developing automatic morphological inflection and analysis tools from under-development IGTs for the Gitksan language, we will discuss how the dynamic nature of linguistic fieldwork has implications/ramifications for expanding the linguistic diversity represented by NLP research (in accordance with the ACL2022 special theme). Through our case-study, we argue that a documentary-linguist-in-the-loop paradigm is essential for every step in developing NLP tools for endangered languages from task specification (Section 3.1) to evaluation (Section 3.4). In particular, we explain how such a paradigm will:
% \begin{itemize}
%     \item Help create computational tasks that will provide the most benefit for documenting and revitalizing endangered languages (Section 3.1)
%   \item Guide research toward more representative/diverse annotation standards for training supervised NLP models (Section 3.2)
%   \item Ensure robustness of NLP systems for several dialects for endangered languages (Section 3.3)
%   \item Prevent harmful overgeneralization of findings and improve adoption of NLP models for language documentation (Section 3.4)
% \end{itemize}












==> edit_2021_11_02/task_specification_3-1.tex <==
% The annotation might be too fine-grained to actually learn from the available data. Might require knowledge about related languages, language history. We might want something that generalizes well, whereas for documentation you might want the most faithful representation. There might be many different uses for the same data and the annotation will typically be a compromise.

% We want to create a resource which is useful for linguists and language learners. It's hard to say what will be useful without consulting end-users.


==> edit_2022_03_12/old_and_notes.tex <==
% But should these languages be considered "left-behind" simply because they lack \textbf{off-the-shelf} datasets for cross-lingual pretraining? Consider a language like Gitksan of the Tsimshianic language family. It has the features of a ``left-behind language'': namely, no off-the-shelf datasets whether unlabeled (e.g., Wikipedia articles) nor labeled (e.g., via the LDC repository\footnote{https://catalog.ldc.upenn.edu}).
% But speakers and linguists have been collaborating to document the language for more than 50 years, producing hours of speech recordings, carefully curated bilingual dictionaries and wordlists, and several thousand tokens of richly-glossed text \citep{forbesetal2017}.   



% \fs{This paragraph needs to be rewritten.}
% Recent work establishes that many NLP tools can be built for low-resource languages based on documentation data such as IGT corpora, with the caveat that this data format has certain idiosyncrasies. We argue that end users in speech communities will not all benefit from a practice of treating IGT corpora as off-the-shelf or standardized datasets due to precisely these idiosyncrasies, which often reflect unique linguistic features arising from novel documentation. We use Gitksan as a case study to illustrate the deficiency of current standards of annotation, model development, and evaluation in this context. Finally, we emphasize the importance of the participation of linguists in the research process surrounding under\-documented languages. 





% \paragraph{Number Marking in Gitksan} %A final major problem that Gitksan's specific morphology poses to the task of paradigm generation is its morphological notion of \textit{plural}.
% Plural in Gitksan has been described as the ``morphological category par excellence'' \cite[52]{rigsby1986}.
% Across both nouns and verbs, plurality and pluractionality can be marked variably by reduplication, affixes, vowel lengthening, suppletion, or some combination of these strategies as demonstrated in Table \ref{tab:plural-examples}. Many lemmas retain a fixed form for singular and plural; others instead have multiple possible forms corresponding to different lexical senses or to different types of pluralization.

% Even though the Unimorph standard incorporates several tags for annotation of grammatical number and these apply readily to both nouns and verbs, the heterogeneity of number marking in Gitksan represents a challenge for the Unimorph schema. 
% %Descriptively, Gitksan plurals are a tangled mess of morphological markers and interpretations which do not neatly map onto one another. 
% On verbs, arguably the major domain of plurality in Gitksan, pluralization indicates either iterative pluractionality or plurality of an absolutive argument (S or P).
% On nouns, it conveys the additive notion of `multiple Ns', but there is some depth to this notion which Gitksan morphology reveals. In Gitksan, additive plurals are usually interpreted in a collective way relative to possession (`multiple Ns owned collectively by the possr(s)'). Distributive plural interpretations (e.g. `multiple Ns, one for each possr') often require specific indication with the morpheme \textit{\Gitg a-}.
% % \todo{GN: As far as I know, Unimorph can only handle this with the use of the partitive / comitative cases, but that's not really what's going on here.}
% Gitksan also allows plural morphemes to stack, conveying multiple types of plurality at once.
% The distributive can be added to a reduplicated plural noun, as in \textit{\Gitg ahumuxw} `ears (pl) (of pl people)', and suppletive plurals are able to optionally reduplicate, perhaps to convey a different or more intense plural interpretation. Unimorph cannot handle stacking of plural markers.

 
%one of three different types of reduplication (CV, CVC, CVx), several different affixes (lV-, \Gitg a-, -xw), vowel lengthening, suppletion, or some irregular combination of these.
%A substantial proportion of 

%The precise plural form of a lemma must be learned on a case by case basis, with no strategy standing out as a clear default.

% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{l|lll}
%     Strategy & Singular & Plural & \\
%     \hline
%         Reduplication & \textit{se'e} & \textit{sise'e} & `leg, foot' \\
%             & \textit{t'is} & \textit{dist'is} & `hit, strike' \\
%             & \textit{gwee'y} & \textit{gwixgwee'y} & `be poor' \\
%         Affixation & \textit{k'uukw} & \textit{\Gitg ak'uukw} & `tail' \\
%              & \textit{aks} & \textit{la'aks} & `drink' \\
%         V Lengthening & \textit{gwila} & \textit{gwiila} & `blanket' \\
%         Irregular & \textit{no\Gitx} & \textit{\Gitg anoona\Gitx xw} & `mother' \\
%              & \textit{\Gitx pts'axw} & \textit{la\Gitx bits'iixw} & `be afraid' \\
%         Suppletion & \textit{t'aa} & \textit{wan} & `sit' \\
%         % Suppletion & ('witxw/bakw, sgi/do\Gitx) \\
%         %  & 
%     \end{tabular}
%     \caption{Gitksan plurals}
%     \label{tab:plural-examples}
% \end{table}

% These examples demonstrate the firmly surface-oriented nature of IGT annotation.
% % In the interlinear-glossed data, most uses of plural affixes are annotated simply as \textsc{pl}, with the exception of the distributive marker, glossed as \textsc{distr}. This surface-oriented annotation is typical for IGT.
% Finer distinctions in meaning might be annotated at a later stage of documentation as the underlying meaning and function of surface morphology is understood. However, UniMorph and UD specifically annotate function, not morphological exponents. This mismatch might lead to substantial reanalysis \todo{[CF: what does this mean? does it mean in the context of trying to interpret IGT through a unimorph lens? does it mean the IGT requires re-annotation?]} of many tokens in the IGT which may be prohibitive.   
% \todo{Is there a proposal about this that can be restated? e.g. impractical to expect less-resourced languages to use unimorph/ud, need to adapt to existing annotation frameworks, this requires collab with linguist. -- also I'd consider swapping this and the previous subsection.} \fs{I agree with CF that we need a concrete proposal about this subsection. Also, I swapped the previous subsections as suggested.}


%From a human or machine learning standpoint, the variety of pluralization strategies and lack of default make the singular-plural alternation difficult to learn. From a pedagogical standpoint, this makes it an invaluable part of any teaching or learning resource. 

%At a semantic level, plural marking is used to convey a variety of interpretations.
% On verbs, arguably the major domain of plurality in Gitksan, pluralization indicates either iterative pluractionality or plurality of an absolutive argument (S or P).
% On nouns, it conveys the additive notion of `multiple Ns', but there is some depth to this notion which Gitksan morphology reveals. In Gitksan, additive plurals are usually interpreted in a collective way under possession (`multiple Ns owned collectively by the possr(s)'). Distributive plural interpretations (e.g. `multiple Ns, one for each possr') often require specific indication with the morpheme \textit{\Gitg a-}. This morpheme sometimes alternates with reduplication, is sometimes appended outside reduplication, or for some lemmas is simply the default means of pluralizing. 



% (ma'us `play' -> mahas'us/mas'us from root `dog', etym: `be like a dog, dog around')


% The same collective versus distributive problem can arise for certain verbal predicates: does the predicate hold of its plural arguments collectively, or of each of them individually?
% Finally, reduplication can be used optionally even on lemmas which are already marked for plural via suppletion, perhaps to augment the existing plural with another interpretation.

 

% Yet, the grammatical properties of Gitksan plurality make it unclear what status it should have as part of a paradigm-level representation.
% Unlike what would typically be expected of inflection, plural and pluractional marking are not totally obligatory; neither are they freely optional.
% In a Gitksan sentence, a plural noun can potentially be indicated in multiple places: the noun itself, the verbal predicate, or any modifier which is derived from a verb.
% % esii ma{\Gitk}di'yhl maaxwsxum gwila
% % esii t'ehldi'yhl mismaaxwsxum gwiila
% So long as plurality is marked on at least one of these elements to convey the meaning, it need not be marked everywhere. That is, there is no obligation to use a plural concord system.
% The obligatoriness of plural marking depends on how it is marked: lemmas with suppletive and irregular plurals are obligatorily marked, while forms involving transparent reduplication are more optional **.
% Furthermore, suppletive plurals are able to optionally reduplicate, perhaps to convey a different or more intense plural interpretation.

% These degrees of optionality and flexibility in plural marking based on the variety of available morphological strategies make it difficult to determine whether plurals should be considered inflectional or derivational.
% Theoretical work on nearby Salish languages, which share some similar properties, has suggested that neither designation is appropriate **.
% It has remained a significant issue for us whether plural forms should be part of the singular lemma's paradigm, or host their own linked paradigms.


For example, the Gitksan morpheme \textit{-xw} has a variety of uses illustrated in example %\fs{Not clear to me which one is inflectional and which derivational} 
\Next, which appear at different points on the scale between more derivation-like (D) to more inflection-like (I).\footnote{The uses include a) creating intransitive predicates from nouns, b) marking inchoatives, c) marking reflexives or passives, d) appearing in the context of certain preverbs, e) appearing optionally in possessives.}

\begin{itemize}
    \item 
\end{itemize}

\ex. 
\a. \textit{os\textbf{xw}}~`have~a~dog' -- \textit{os}~`dog' (D)
\b. \textit{mit\textbf{xw}}~`be~full' -- \textit{midin}~`fill' (D)
\b.  \textit{jap\textbf{xw}}~`be~made' -- \textit{jap}~`do,~make' (D?)
\b. \textit{sik'ihl~huut\textbf{xw}}~`try~to~run~away' \\-- \textit{huut}~`run~away' (I?)
\b. \textit{la\Gitx yip\textbf{xw}si'm} `your (pl) land' \\-- \textit{la\Gitx yipsi'm} `your (pl) land' (?)



%  In a step to achieve this, we strongly recommend usage of Model Cards \citep{Mitchell2019ModelCF} for NLP research projects on under\-documented languages. \todo{CF: what are model cards? did we use them? are these meant to be used iteratively throughout the project?} In employing Model Cards, we can ask questions relevant to NLP research in under\-documented languages including: How did the limited dialectal/speaker coverage affect modelling choices? What is the dialect coverage of the dataset used in this project? Were any dialects left out? Does the dataset reflect a diverse set of speakers? Do the selected evaluation methods adequately represent practical use-cases of the model? Are there plans for the speaker community to benefit from this research? \todo{cf: it sounds like they are more introspective questions than prompts for collaboration so this recommendation doesn't seem to exactly align with paper's goal} \fs{That's true; maybe we can take that part out. Not sure what else we can put here. Maybe discussion of evaluation metrics in NLP research?}
%     \item How did the limited dialectal/speaker coverage affect modelling choices?
% \begin{itemize}
%     % \item Is this dataset representative of all dialects? Which ones does it represent?
%     \item What is the dialect coverage of the dataset used in this project? Were any dialects left out?
%     \item Does the dataset reflect a diverse set of speakers?
%     \item How did the limited dialectal/speaker coverage affect modelling choices?
%     % \item If our datasets are not representative of the dialectal variety in the target language, or we have data from very few speakers, how will this affect our modeling choices?
%     \item Do the selected evaluation methods adequately represent practical use-cases of the model?
%     \item Are there plans for the speaker community to benefit from this research? 
% \end{itemize}
